Graphs, Entities, and Step Mixture

Existing approaches for graph neural networks commonly suffer from the oversmoothing issue, regardless of how neighborhoods are aggregated. Most methods also focus on transductive scenarios for fixed graphs, leading to poor generalization for unseen graphs. To address these issues, we propose a new graph neural network that considers both edge-based neighborhood relationships and node-based entity features, i.e. Graph Entities with Step Mixture via random walk (GESM). GESM employs a mixture of various steps through random walk to alleviate the oversmoothing problem, attention to dynamically reflect interrelations depending on node information, and structure-based regularization to enhance embedding representation. With intensive experiments, we show that the proposed GESM achieves state-of-the-art or comparable performances on eight benchmark graph datasets comprising transductive and inductive learning tasks. Furthermore, we empirically demonstrate the significance of considering global information.

==> 07.related.tex <==

For transductive learning, we compare our model with numbers of state-of-the-art models according to the results reported in the corresponding papers. Our model is compared with baseline models specified in~\citep{velivckovic2017graph} such as label propagation (LP)~\citep{xiaojin2002learning}, graph embeddings via random walk (DeepWalk)~\citep{perozzi2014deepwalk}, and Planetoid~\citep{yang2016revisiting}. We also compare our model with models that use self-supervised learning (Union)~\citep{li2018deeper}, learnable graph convolution (LGCN)~\citep{gao2018large}, GCN based multi-hop neighborhood mixing (JK-GCN and MixHop)~\citep{xu2018representation, abu2019mixhop}, multi-scale graph convolutional networks (AdaLNet)~\citep{liao2019lanczosnet} and hyperbolic graph convolution network (HGCN)~\citep{chami2019hyperbolic}. We further include models that utilize teleport term during propagation APPNP~\citep{klicpera2018predict}, conduct convolution via spectral filters such as ChebyNet~\citep{defferrard2016convolutional}, GCN~\citep{kipf2016semi}, SGC~\citep{wu2019simplifying}, and GWNN~\citep{xu2019graph} and models that adopt attention between nodes, such as GAT~\citep{velivckovic2017graph} and AGNN~\citep{thekumparampil2018attention}. 

For inductive learning tasks, we compare our model against four baseline models. This includes graphs that use sampling and aggregation (GraphSAGE-LSTM)~\citep{hamilton2017inductive}, and jumping-knowledge (JK-LSTM)~\citep{xu2018representation}, along with GAT and LGCN which are used in the transductive setting. 

